A Performance Analysis of Task Scheduling for UQ Workflows on HPC Systems

Uncertainty Quantification (UQ) workloads are becoming increasingly common in science and engineering. They involve the submission of thousands or even millions of similar tasks with potentially unpredictable runtimes, where the total number is usually not known a priori. A static one-size-fits-all batch script would likely lead to suboptimal scheduling, and native schedulers installed on High Performance Computing (HPC) systems such as SLURM often struggle to efficiently handle such workloads. In this paper, we introduce a new load balancing approach suitable for UQ workflows. To demonstrate its efficiency in a real-world setting, we focus on the GS2 gyrokinetic plasma turbulence simulator. Individual simulations can be computationally demanding, with runtimes varying significantly-from minutes to hours-depending on the high-dimensional input parameters. Our approach uses UQ and Modelling Bridge, which offers a language-agnostic interface to a simulation model, combined with HyperQueue which works alongside the native scheduler. In particular, deploying this framework on HPC systems does not require system-level changes. We benchmark our proposed framework against a standalone SLURM approach using GS2 and a Gaussian Process surrogate thereof. Our results demonstrate a reduction in scheduling overhead by up to three orders of magnitude and a maximum reduction of 38% in CPU time for long-running simulations compared to the naive SLURM approach, while making no assumptions about the job submission patterns inherent to UQ workflows.

==> abstract <==
# Parallel computing track
Efficient scheduling on high-performance computing (HPC) systems is critical for optimizing resource utilization. Traditional schedulers, such as SLURM and PBS, are poorly suited for workloads involving many small, loosely coupled tasks, common in uncertainty quantification (UQ). These workloads often require running thousands of simulations with varying input parameters, leading to high scheduling overhead and suboptimal resource use. This paper presents a scheduling approach for UQ workloads using the UM-Bridge framework and HyperQueue (HQ). The method integrates with existing HPC schedulers without requiring system-level changes, enabling easier adoption by domain specialists. We benchmark the approach using two applications: GS2, a gyrokinetic plasma turbulence simulator, and a Gaussian Process surrogate. Results show that our approach reduces scheduling overhead and improves makespan efficiency compared to SLURM, particularly for short jobs.


# Applications Track
Efficient scheduling on high-performance computing (HPC) systems is critical for workloads involving many small, loosely coupled tasks, such as those common in uncertainty quantification (UQ). This paper focuses on the gyrokinetic plasma turbulence simulator GS2, which models plasma behavior in fusion reactors by solving the Vlasov-Maxwell system. Individual simulations are computationally expensive and have strongly varying runtimes, from minutes to hours, in dependence of high-dimensional input parameters. For parameter exploration tasks we require thousands of simulations, leading to high scheduling overhead and suboptimal resource use. Traditional schedulers, such as SLURM or PBS, struggle to efficiently manage these workloads.  We propose an alternative scheduling approach using the UM-Bridge framework with HyperQueue (HQ). This method integrates with existing HPC schedulers without system-level change. Benchmarks compare the performance of our approach to a purely SLURM based solution for gyrokinetic plasma simulations and their Gaussian Process surrogates.
Results show HQ reduces scheduling overhead and improves makespan efficiency, particularly for shorter tasks, as measured by the Scheduler Length Ratio (SLR). These findings demonstrate our approaches suitability for workloads with vastly varying runtimes and large numbers of loosely connected tasks.



# Conclusions

In this paper, we applied the UM-Bridge HQ framework to realistic workloads from a gyrokinetic plasma application and compared its performance with the traditional SLURM scheduler on our local HPC system Hamilton8. Our results show that the HQ-based approach either outperforms or is comparable to SLURM. This improvement is primarily due to reduced scheduling overhead, which is up to 3 orders of magnitude lower than that of a pure SLURM submission. We emphasize that the framework is not restricted to the examples presented and can be adapted to a wide range of applications with similar characteristics, including loosely-coupled, parallel tasks.

There are several potential areas for architectural improvement. For jobs with rapid execution times, we propose the introduction of dedicated model servers that could offload processing to GPUs or other accelerators. These servers would be used only to handle surrogate evaluations, rather than conflicting with possibly concurrent submissions of full forward model evaluations. This allows HQ to more efficiently schedule these extremely fast running jobs. The UM-Bridge wrapper is not needed in this case, removing the 1 second overhead it introduces. To address issues related to filesystem dependencies, we also plan to implement a network-based method for relaying information such as IP addresses and port numbers. 

The main area for future exploration is the extension of the framework to handle more complex workflows, where tasks have interdependencies or dynamic scheduling requirements. For example, tasks that evaluate integrals or perform Bayesian inference may require multiple stages of computation, with each stage dependent on the results of the previous. 

# Abstract next iteration

Uncertainty Quantification (UQ) workloads are becoming increasingly important in many fields of science and engineering. They involve the submission of thousands or even millions of of similar tasks, in many cases with dynamic scheduling requirements. Native schedulers installed on High-Performance Computing (HPC) systems such as SLURM or PBS often struggle to efficiently handle such workloads.
In this paper we introduce a new load balancing approach suitable for UQ workflows. To demonstrate its efficiency in a real world setting we focus on the gyrokinetic plasma turbulence simulator GS2, which models plasma behaviour in fusion reactors by solving the Vlasov-Maxwell system. Individual simulations can be computationally demanding, with runtimes varying significantly—from minutes to hours—depending on the high-dimensional input parameters. Our scheduling approach uses UM-Bridge (the UQ and Modeling Bridge), which offers an interface to a simulation model, combined with HyperQueue (HQ) as the meta-scheduler working on top of the native scheduler. Notably, deploying this framework on HPC systems does not require system-level changes. We benchmark our load balancer against a standalone SLURM approach using GS2 and a Gaussian Process (GP) surrogate theoref. Our results indicate that our appraoch reduces scheduling overheads by up to three orders of magnitude across the benchmarks, thus improving the scheduling efficiency as measured by the Schedule Length Ratio (SLR). We reach a maximum reduction of 38\% in CPU time for long-running submissions.
